State-Compute Replication: Parallelizing High-Speed Stateful Packet Processing

With the slowdown of Moore's law, CPU-oriented packet processing in software will be significantly outpaced by emerging line speeds of network interface cards (NICs). Single-core packet-processing throughput has saturated. We consider the problem of high-speed packet processing with multiple CPU cores. The key challenge is state--memory that multiple packets must read and update. The prevailing method to scale throughput with multiple cores involves state sharding, processing all packets that update the same state, i.e., flow, at the same core. However, given the heavy-tailed nature of realistic flow size distributions, this method will be untenable in the near future, since total throughput is severely limited by single core performance. This paper introduces state-compute replication, a principle to scale the throughput of a single stateful flow across multiple cores using replication. Our design leverages a packet history sequencer running on a NIC or top-of-the-rack switch to enable multiple cores to update state without explicit synchronization. Our experiments with realistic data center and wide-area Internet traces shows that state-compute replication can scale total packet-processing throughput linearly with cores, deterministically and independent of flow size distributions, across a range of realistic packet-processing programs.

==> eval-conntrack-tokenbucket-different-packetsizes-mlffr.tex <==
\begin{figure}
  \vspace{-5mm}
  \centering
  \subfloat[Fixed pkt size (conntrack)]{
    \begin{minipage}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{figs/eval/dctcp/xdp_conntrack_mlffr.pdf}
    \label{fig:throughput-conntrack-dctcp}
    \vspace{-4mm}
    \end{minipage}}
  \subfloat[Varying pkt size (token bucket)]{
    \begin{minipage}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{figs/eval/univ1_64B_nopadding/xdp_token_bucket_mlffr.pdf}
    \label{fig:throughput-external-mlffr-tokenbucket}
    \vspace{-4mm}
  \end{minipage}}
  \vspace{-2.5mm}
  \caption{
    (a) Comparing the throughput of a TCP connection state tracker
    parallelized using three techniques, SCR (\Sec{design}), shared
    state and sharding (\Sec{motivation-background}) on the
    hyperscalar data center trace (\Sec{eval-experiment-setup}). The
    packet sizes used by all baselines is the same.
    (b) Comparing the throughput of a token bucket policer
    parallelized using the same three techniques on the university
    data center trace (\Sec{eval-experiment-setup}), while truncating
    all packets in the trace to 64 bytes, and having only \SCR add
    metadata to packets before feeding them to the NIC.
 }
    \label{fig:throughput-numbers-assorted}
    \vspace{-6mm}
\end{figure}


==> eval-rss++.tex <==
\begin{figure}
  %%\vspace{-5mm}
  \centering
  \includegraphics[width=0.25\textwidth]{figs/eval/dctcp/xdp_conntrack_rsspp_far_numa.pdf}
  \vspace{-2mm}
  \caption{Comparing TCP connection tracking
    parallelized using \SCR and RSS++~\cite{rss++-conext19} on the
    hyperscalar data center trace (\Sec{eval-experiment-setup}). }
  \vspace{-6mm}
  \label{fig:throughput-rsspp}
\end{figure}


==> eval-trace-throughput-conntrack-graph.tex <==
\begin{figure}
  %%\vspace{-5mm}
  \centering
  \includegraphics[width=0.25\textwidth]{figs/eval/dctcp/xdp_conntrack_mlffr.pdf}
  \vspace{-2mm}
  \caption{Comparing the throughput of a TCP connection state tracker
    parallelized using three techniques, SCR (\Sec{design}), shared
    state and sharding (\Sec{motivation-background}) on the
    hyperscalar data center trace (\Sec{eval-experiment-setup}).}
  \vspace{-6mm}
  \label{fig:throughput-conntrack-dctcp}
\end{figure}


==> eval-trace-throughput-external-mlffr.tex <==
\begin{figure}
  %%\vspace{-5mm}
  \centering
  \includegraphics[width=0.25\textwidth]{figs/eval/univ1_64B_nopadding/xdp_token_bucket_mlffr.pdf}
  \vspace{-2mm}
  \caption{Comparing the throughput of a token bucket policer
    parallelized using three techniques, SCR (\Sec{design}), shared
    state and sharding (\Sec{motivation-background}) on the university
    data center trace (\Sec{eval-experiment-setup}), while truncating
    all packets in the trace to 64 bytes. Only \SCR adds metadata to
    packets before being fed into the NIC. %% consuming more NIC
    %% bandwidth and PCIe bandwidth, and incurring additional L3 cache
    %% pressure. Beyond 9 cores, the bottleneck is no longer the CPU, and
    %% the performance gains from \SCR saturate, while its throughput
    %% continues to remain much higher than the other baselines.
  }
  \vspace{-6mm}
  \label{fig:throughput-external-mlffr-tokenbucket}
\end{figure}



==> extra.tex <==
%\begin{wrapfigure}{r}{0.50\textwidth}
\begin{figure}
  \vspace{-5mm}
  \centering
  \subfloat[A port-knocking firewall]{
    \begin{minipage}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{figs/avg_rx_rate_portknock.pdf}
    \label{fig:thoughput-portknock}
    %%\vspace{-4mm}
    \end{minipage}} 
    % \hspace{0.01\textwidth}%
  \subfloat[Heavy hitter detector]{
    \begin{minipage}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{figs/avg_rx_rate_heavyhitter.pdf}
    \label{fig:thoughput-heavyhitter}
    %%\vspace{-4mm}
    \end{minipage}}
    %%\vspace{-2.5mm}
    \caption{Throughput (millions of packets per second) of two
      stateful packet-processing programs implemented using our scaling
      principles (termed ``shared nothing'' in the graph) and through
      explicit synchronization (termed ``shared state''). Error bars
      denote standard deviations. In these experiments, every packet
      touches the same state, hence state sharding approaches are
      limited by single-core throughput, captured by the points where
      the number of cores $= 1$.}
    \label{fig:throughput}
    \vspace{-5mm}
\end{figure}
%%\end{wrapfigure}

\Para{Preliminary experimental results: Do scaling principles work?}
We implemented two stateful packet-processing programs in eBPF and
attached them to the NIC device driver ({\ct xdp}~\cite{xdp-conext18}
hook). These programs implement a port-knocking
firewall~\cite{port-knocking-firewall} and a heavy hitter detector. We
set up each of these programs to update a {\em single shared state}
across all packets. For port knocking, we implemented two variants of
the program, one that uses our scaling principles (``shared nothing'')
and another using explicit synchronization across cores with
fine-grained locking (``shared state''). For the heavy-hitter
application, we implemented the above variants, as well a third
version that uses hardware-optimized transactional memory operations
to update shared state across cores. A state sharding approach on this
workload will send all packets to the same core since all packets
update the same state.

To evaluate how packet-processing throughput (packets-per-second)
scales with the number of cores, we use two servers on
CloudLab~\cite{cloudlab} to set up a high-speed packet generator using
TRex and a Device Under Test (DUT). Each server has 10-core Intel
Broadwell (E5-2640v4) 2.4 GHz processors with a PCIe 3.0 bus and 64 GB
of memory, and is equipped with two Mellanox ConnectX-4 25Gbps
NICs. The traffic generator piggybacks recent packet history while
sending packets into the DUT at line rate.
%
\cut{
The packets are processed
by the DUT and forwarded back to the packet generator.
}
%
\Fig{throughput} shows that the throughput when using the scaling
principles scales linearly with the number of cores for both
applications, until it hits the line rate of the NIC (in
packets-per-second). In contrast, state sharding is limited by
single-core throughput, and synchronization-based approaches scale
much poorer in comparison.








\nop{
  \begin{figure*}[ht]
    \centering
    \[
    \begin{array}{ccc}
    \includegraphics[width=0.31\textwidth]{figs/xdp_fwd_avg_rx_rate.pdf} &
    \includegraphics[width=0.31\textwidth]{figs/xdp_fwd_avg_rx_rate_Gbps.pdf} &
    \includegraphics[width=0.31\textwidth]{figs/xdp_fwd_avg_latency_ns.pdf}\\

    \mbox{(a) Throughput (packets/second)} & \mbox{(b) Throughput
      (bytes/second)} & \mbox{(c) Computation latency (nanoseconds)}
    \\
    
  \end{array}
  \]
    \caption{The nature of CPU work in high-speed packet processing:
      Consider the throughput of a simple packet forwarding
      application (packets/second (a), bytes/second (b)) running on a
      single CPU core clocked at 3.6 GHz, as the size of the incoming
      packets varies.  The average latency to execute the XDP program
      is also shown in nanoseconds (c). CPU usage is tied to the
      number of packets processed per second, not the bytes processed
      per second. Further, significant time elapses in {\em dispatch:}
      CPU work needed to present the input packet to and retrieve the
      output packet from the ``interesting'' packet-processing
      computation.}
    \label{fig:nature-of-packet-processing-cpu-work}
  \end{figure*}
}


==> parallel-cpu-programming.tex <==
%% \subsection{\SCR-Aware Multi-Core Programming}
%% \label{sec:scr-programming}

%% CONTENTS of this section have been fully moved to the appendix.


==> throughput-model-large-cores.tex <==
\begin{figure}
  %%\vspace{-5mm}
  \centering
  \includegraphics[width=0.25\textwidth]{figs/throughput_model/throughput_model_cores.pdf}
  \vspace{-2mm}
  \caption{xxxx}
  \vspace{-6mm}
  \label{fig:throughput-model-cores}
\end{figure}


==> xdp-portknock-metadata-structure.tex <==
\begin{lstlisting}
struct meta {
  int l3proto;
  int l4proto;
  int srcip;
  int dport;
}
\end{lstlisting}

